Automated Repair of Unrealisable LTL Specifications Guided by Model Counting

The reactive synthesis problem consists of automatically producing correct-by-construction operational models of systems from high-level formal specifications of their behaviours. However, specifications are often unrealisable, meaning that no system can be synthesised from the specification. To deal with this problem, we present AuRUS, a search-based approach to repair unrealisable Linear-Time Temporal Logic (LTL) specifications. AuRUS aims at generating solutions that are similar to the original specifications by using the notions of syntactic and semantic similarities. Intuitively, the syntactic similarity measures the text similarity between the specifications, while the semantic similarity measures the number of behaviours preserved/removed by the candidate repair. We propose a new heuristic based on model counting to approximate semantic similarity. We empirically assess AuRUS on many unrealisable specifications taken from different benchmarks and show that it can successfully repair all of them. Also, compared to related techniques, AuRUS can produce many unique solutions while showing more scalability.

==> ltl-model-counting.tex <==
\section{Model Counting for LTL}
\label{sec:ltl-model-counting}

Related to the satisfiability problem, the \emph{model counting} problem (\#SAT) consists of counting how many models satisfy a given formula. In the case of LTL, \#SAT consists of counting the number of traces that satisfy an LTL formula $\varphi$. 
Notice that, the number of models is zero when the formula is unsatisfiable. But, if $\varphi$ is satisfiable, then an \emph{infinite} number of models satisfying $\varphi$  can be generated (e.g., new models can be built by unfolding a satisfying model any finite number of times). 
In order to obtain a more significant value, \#SAT for LTL is usually restricted to \emph{bounded models}. Given a bound $k$, the \#SAT problem consists of calculating how many models of at most $k$ states exist. Recalling the LTL semantics (Section~\ref{sec:ltl}), models for  LTL formulas are characterised by \emph{lasso traces} \cite{Finkbeiner+2014}, which are represented as a finite sequence of states, called the \emph{base} of the trace, such that the last state has a loop to some previous state.   
Fig.~\ref{fig:lasso-trace} is an example of a lasso trace that satisfies the LTL formula $\G(p \Implies \X q)$.
%Formally, given a set $AP$ of atomic propositions, a word model $\sigma$ is a sequence of states $s_0,\ldots,s_{i-1},(s_i,\ldots,s_k)^\omega$, such that, $s_0,\ldots,s_k \in 2^{AP}$; in such a word model, there is a loop from state $k$ to state $i$.  

\vspace{-1em}
\begin{figure}[htp]
\begin{minipage}[t]{0.41\textwidth}
\centering
\includegraphics[scale=.45]{lasso-traces.pdf}
\caption{Lasso trace for $\G(p \Implies \X q)$.}
\label{fig:lasso-trace}
\end{minipage}\hspace*{.2em}
\begin{minipage}[t]{0.3\textwidth}
\centering
\includegraphics[scale=.4]{dfa.pdf}
\caption{Finite automaton.}% for $\G(p \lor q)$.}
\label{fig:dfa}
\end{minipage}%\hspace*{.5em}
\begin{minipage}[t]{0.3\textwidth}
\centering
\includegraphics[scale=.45]{transfer-matrix.pdf}
\caption{Transfer matrix.}% $\G(p \lor q)$.}
\label{fig:transfer-matrix}
\end{minipage}
\end{figure}
\vspace{-1em}

Unfortunately, currently there is no approach to solve efficiently \#SAT for general LTL formulas.
Particularly, the approach presented in \cite{Finkbeiner+2014} is very efficient to solve \#SAT for safety properties, but it does not apply to liveness formulas, the ones we target in this work. On the other hand, one can think to employ a bounded model checking like approach~\cite{Biere+1999}, that consists of reducing LTL formulas, for a given bound, to propositional formulas, and then use any model counter for propositional logic (e.g., \texttt{ganak}~\cite{Sharma+2019}) for indirectly computing \#SAT for LTL. 
However, as it was shown in \cite{Finkbeiner+2014}, while the bound is incremented, the propositional constraints generated by this translation become intractable by the available model counters. 

Recently, an approach for approximating the model counting problem for LTL has been presented in \cite{Degiovanni+2018}. Intuitively, from a given LTL formula $\varphi$, it first generates a regular expression $e_\varphi$, that represents the prefixes accepted by $\varphi$. Then, a string model counter is employed to compute how many strings, up to a bounded length, are recognized by the regular expression $e_\varphi$. This number is used to estimate the number of models that satisfy $\varphi$. 
It is worth to mention that, to solve the just mentioned model counting problem, \cite{Degiovanni+2018} uses an automata-based string model counter, namely, ABC~\cite{Aydin+2015}. Basically, ABC takes as input a regular expression $e$, and then produces an equivalent automaton $A_e$, such that, the strings accepted by $A_e$ are guaranteed to satisfy the regular expression $e$. 
The success of ABC relies on the very efficient representation of the automaton $A_e$ as a transfer matrix $T_e$, enabling the use of matrices operations to indirectly solve the string model counting problem, something that can be very fast computed by modern libraries.  

In this work, we estimate the number of models of an LTL formula $\varphi$, by first generating an automaton representation $A_\varphi$, such that, the paths recognised by $A_\varphi$ are the base of some lasso trace satisfying $\varphi$. Then, we encode this automata into a transfer matrix $T_\varphi$, in order to indirectly solve the LTL model counting problem, by matrices operations, in the same way as ABC does.

Precisely, given the LTL formula $\varphi$, we generate the transfer matrix $T_\varphi$ by performing the following tree encodings: (1) we generate the B\"uchi automaton $B_\varphi$ that recognises $\varphi$; (2) we generate a Finite State Automaton $A_\varphi$ from $B_\varphi$; and (3) we generate the transfer matrix $T_\varphi$ from $A_\varphi$.
Intuitively, the B\"uchi automaton $B_\varphi$ recognises all the lasso traces satisfying $\varphi$. Recall that B\"uchi automata recognise infinite traces, since their accepting condition requires that some accepting state has to be visited infinitely often in the lasso trace. 
On the contrary, finite automata recognise finite traces, since their accepting condition requires only reaching some final state.
Then, when we generate the finite automaton $A_\varphi$ from $B_\varphi$, the finite traces recognised by $A_\varphi$ will be part of some lasso trace recognised by $B_\varphi$. 
Finally, we encode $A_\varphi$ into a $N \times N$ transfer matrix $T_\varphi$, where $N$ is the number of states in $A_\varphi$, such that, the value of each $T_\varphi[i,j]$ denotes the number of transitions from state $i$ to state $j$.  
Thus, the number of traces of length $k$ accepted by $A_\varphi$, can be computed using matrix multiplication.
We compute $I \times T_{\varphi}^{k} \times F$, where: $I$ is a row vector codifying the initial states; $T_{\varphi}^{k}$ is the matrix resulting from multiplying $k$ times matrix $T_{\varphi}$; and $F$ is a column vector codifying the final states of $A_\varphi$. 
Precisely, $I[1,j] = 1$ if and only if $j$ is a initial state, and $0$ otherwise; and $F[i,1] = 1$ if and only if $i$ is a final state, and $0$ otherwise. 

For instance, Fig.~\ref{fig:dfa} and Fig.~\ref{fig:transfer-matrix} show the finite automaton and the transfer matrix, respectively, generated by our approach from the LTL formula $\G(p \Implies \X q)$. Then, considering the bound $k$ equals to $4$, our model counting  approach answers that there are 108 models, computed by the following matrices multiplication:
\[
I\times T_\varphi^4 \times F =
\begin{bmatrix}
    1  &  0  &  0  \\   
\end{bmatrix}
\times 
\begin{bmatrix}
    0  & 2  &  2  \\
    0  & 1  &  1  \\
    0  & 2  &  2  \\     
\end{bmatrix}^4
\times
\begin{bmatrix}
	0	\\
    1   \\
    1      
\end{bmatrix}
=
\begin{bmatrix}
    1  &  0  &  0  \\   
\end{bmatrix}
\times 
\begin{bmatrix}
    0  & 54  &  54  \\
    0  & 27  &  27  \\
    0  & 54  &  54  \\
\end{bmatrix}
\times
\begin{bmatrix}
    0	\\
    1   \\
    1        
\end{bmatrix}
= 108
\]

Notice that, there exists exactly 351 lasso traces for $\G(p \Implies \X q)$, but our approach reports only 108 (i.e., the number of bases for these traces). However, we will use this value in our fitness function as a indirect measure to compare the number of models of different specifications. That is, given two formulas $\varphi$ and $\psi$, and a bound $k$, if our approach returns that $\#(\varphi, k) > \#(\psi, k)$, we will assume that this relation would be preserved, if we were able to compute the precise number of models for each formula. Then, our search-based algorithm uses this measure to rank the candidate specifications refinements. We show empirical evidence of this assumption in Section~\ref{sec:validation}. 

During all the process, our approach employs different libraries to manipulate automata and matrices. 
Precisely, we use OWL~\cite{Kretinsky+2018} to translate LTL formulas to B\"uchi, JFLAP~\cite{JFLAP}to minimize and determinize the finite automata, and EJML~\cite{EJML} to manipulate the matrices.



